Online Budgeted Allocation with General Budgets

We study the online budgeted allocation (also called ADWORDS) problem, where a set of impressions arriving online are allocated to a set of budget-constrained advertisers to maximize revenue. Motivated by connections to Internet advertising, several variants of this problem have been studied since the seminal work of Mehta, Saberi, Vazirani, and Vazirani (FOCS 2005). However, this entire body of work focuses on a single budget for every advertising campaign, whereas in order to fully represent the actual agenda of an advertiser, an advertising budget should be expressible over multiple tiers of user-attribute granularity. A simple example is an advertising campaign that is constrained by an overall budget but is also accompanied by a set of sub-budgets for each target demographic. In such a contract scheme, an advertiser can specify their true user-targeting goals, allowing the publisher to fulfill them through relevant allocations. In this paper, we give a complete characterization of the ADWORDS problem for general advertising budgets. In the most general setting, we show that, unlike in the single-budget ADWORDS problem, obtaining a constant competitive ratio is impossible and give asymptotically tight upper and lower bounds. However for our main result, we observe that in many real-world scenarios (as in the above example), multi-tier budgets have a laminar structure, since most relevant consumer or product classifications are hierarchical. For laminar budgets, we obtain a competitive ratio of e/(e-1) in the small bids case, which matches the best known ADWORDS result for single budgets. Our algorithm has a primal-dual structure and generalizes the primal-dual analysis for single- budget ADWORDS first given by Buchbinder, Jain, and Naor (ESA 2007).

==> ec-mm-laminar-large.tex <==
%\section{Analysis of Greedy Algorithm for \lam with arbitrary bids} 
%\label{append:lamgreedy}

\subsection{General bids}
\label{subsec:lam-large}
We now prove the second part of Theorem \ref{thm:lam} by showing that for \lam, 
the greedy algorithm is $2$-competitive with arbitrary bids. 
As in Section \ref{subsec:lam-sb}, we again do a primal-dual analysis. However, we will now use the  
original dual formulation $D$, since in this analysis, we will observe which budgets became tight at the end of the instance 
and set the corresponding $\alpha_u^{(s)}$ variables accordingly. (In other word, we use a dual fitting analysis rather than  primal dual algorithm). 
Recall the original dual formation, given as follows. 

\begin{gather}
\min \sum_u \sum_{s \in S_u} \alpha_{u}^{(s)} B_{u}^{(s)} + \sum_v \sigma_v \label{eq:odual1} \\ 
\forall \ u \in U,~ v \in V,~  t \subseteq K : \quad  \sum_{s \in S_u} \left(\alpha_{u}^{(s)} \sum_{k \in K_s} r_{uvt}^{(k)}\right)  + \sigma_v \geq \sum_{k} r_{uvt}^{(k)}\label{eq:odual2} \\
\forall \ u \in U,~ s\in S_u: \quad  \alpha_{u}^{(s)} \geq 0 \notag. 
\end{gather} 

Again let $F_u$ be the forest that represents
the laminar set system $S_u$.
We set our dual variables $\alpha_u^{(s)}$ and $\sigma_v$ as follows.
\begin{itemize} 
\item Let $R_v$ be the total revenue earned by the algorithm from assigning impression $v$. Then we 
set $\sigma_v = R_v$. Note that if algorithm only earns some fraction of the revenue generated from the impression (because the total revenue exceeds 
the remaining budget capacity), then the algorithm 
\item At the end of the algorithm, for each budget $B_{u}^{(s)}$ that is at capacity and none of its ancestor budgets in $F_u$ 
are at capacity, we set $\alpha_u^{(s)} = 1$ 
(all other $\alpha_u^{(s)}$ are set to be 0). 
\end{itemize}  

It suffices to show that the constructed dual is feasible and has 
cost at most twice of that earned by the algorithm. \\ 

%Recall the objective of dual $D$: 
%\begin{equation*}
%\min \sum_{u, \in U, s \in S_u} \alpha_{u}^{(s)} B_{u}^{(s)} + \sum_v \sigma_v .
%\end{equation*} 


\noindent {\bf Primal-Dual Ratio:} We now show a ratio of 2 between the dual and primal objectives (the former given by Eqn.\ \eqref{eq:odual1}).  
Clearly $\sum_{v \in V} R_v = \sum_{v \in V} \sigma_v$ equals the total revenue earned by the greedy algorithm. 
The former term in the objective, $\sum_{u, \in U, s \in S_u} \alpha_{u}^{(s)} B_{u}^{(s)}$, will amount to the total capacity of saturated budgets 
that do not have tight ancestors in $F_u$.  This also upper bounds the total revenue earned by the algorithm, since for each dimension $k$ and bidder $u$, 
revenue earned on $k$ from $u$ is counted in this total by the saturated budget of at most one of the ancestor sets
of constraint $\{k\}$ (in other words, $k$ can belong to at most one maximal saturated budget set $K_s$).  Thus, the objective of the dual is at most twice the 
revenue of the algorithm.  \\ 

%Recall the constraints in $D$ are given by: 
%\begin{equation*} 
%\forall \ u \in U, v \in V,  t \subseteq: K: \sum_{s \in S_u} \left(\alpha_{u}^{(s)} \sum_{k \in s} r_{uvt}^{(k)}\right)  + \sigma_v \geq \sum_{k} r_{uvt}^{(k)}. \notag \\
%\end{equation*} 


\noindent {\bf Feasibility:}  We now show dual feasibility (i.e., Eqn.\ \eqref{eq:odual2} holds). 
Note that assignment types where $t \neq K$ will only make the inequality easier to satisfy (dimensions $k$ not included in type $t$
contribute $r_{uvt}^{(k)} = 0$ to both sides of the inequality). Therefore for simplicity, we will assume $t = K$. 

Let $R_v^{(u)}$ be the revenue that algorithm would have earned from the impression $v$ if the algorithm had assigned it to $u$, i.e., the sum of $r_{uv}^{(k)}$ for 
all active dimensions $k$ when $v$ arrived.  Since the algorithm assigns greedily, clearly $R_v^{(u)} \leq R_v = \sigma_v$.  Therefore, for the inequality to 
hold, it suffices to show $\sum_{s \in S_u} \left(\alpha_{u}^{(s)} \sum_{k \in s} r_{uvt}^{(k)}\right)$ is at least the sum of revenues from inactive dimensions when 
impression $v$ arrived. However, this follows directly from how we set $\alpha_u^{(s)}$: if a dimension $k$ is 
inactive when $v$ arrives, it must have at least one tight ancestor constraint in $F_u$. 
This implies that at the end of the algorithm, there will be at least one ancestor $s'$ of dimension $k$ in $F_u$ where we will set $\alpha_u^{(s')} = 1$, 
which then contributes the desired $r_{uv}^{(k)}$ term to the LHS of the inequality.  

